Mini-Proceedings of the "Fourth International Workshop on the Extension Project for the J-PARC Hadron Experimental Facility (HEF-ex 2024)"

The mini proceedings of the "Fourth International Workshop on the Extension Project for the J-PARC Hadron Experimental Facility (HEF-ex 2024) [https://kds.kek.jp/event/46965]" held at J-PARC, February 19-21, 2024, are presented. The workshop was devoted to discussing the physics case that connects both the present and the future Hadron Experimental Facility at J-PARC, covering a wide range of topics in flavor, hadron, and nuclear physics related to both experimental and theoretical activities being conducted at the facility.

==> Yu/diphoton-GPD_orig.tex <==
The high-energy pion beam at J-PARC allows to probe hadron structures by extracting generalized parton distributions (GPDs)
through the hard exclusive diphoton production process~\cite{Qiu:2022bpq, Qiu:2024mny},
\beq[eq:diphoton]
	N(p) + \pi(p_2) \to N'(p') + \gamma(q_1) + \gamma(q_2),
\eeq
where the nucleon $N$ is diffracted to $N'$ in the near-forward direction.
This process is conveniently analyzed in the center-of-mass frame of the final-state photons, 
with the pion moving along the $-\hat{z}$ direction and the nucleons lying on the $\hat{x}$-$\hat{z}$ plane,
as shown in \fig{fig:frame} where the angles $\theta$ and $\phi$ of the photons are also defined.
In the kinematic region where the nucleon momentum transfer $t = (p - p')^2$ is much smaller than the transverse momenta of the final-state photons,
\beq
	q_T = |\bm{q}_{1T}| = |\bm{q}_{2T}| \gg \sqrt{|t|},
\eeq
the amplitude of \eq{eq:diphoton} can be factorized into nucleon transition GPDs $F^{[q\bar{q}']}_{NN'}(x,\xi,t)$ and $\wt{F}^{[q\bar{q}']}_{NN'}(x,\xi,t)$ 
and pion distribution amplitude $D^{[q'\bar{q}]}_{\pi}(z)$, 
convoluted with perturbatively calculable hard coefficients,
\begin{align}
	\mathcal{M}(\xi, t, \theta)
	&= \int_{-1}^{1} dx \int_0^1 dz \, D^{[q'\bar{q}]}_{\pi}(z) 
		\bb{ \wt{F}^{[q\bar{q}']}_{NN'}(x,\xi,t) \, C(x, \xi; z; \theta)				
			+ F^{[q\bar{q}']}_{NN'}(x,\xi,t) \, \wt{C}(x, \xi; z; \theta)
		}, 
\label{eq:factorize}
\end{align}
up to corrections suppressed by powers of $\sqrt{|t|} / q_T$.
Since only charged pion beams are accessible in experiments, the nucleon diffraction involves a flavor transition, 
with $(NN') = (pn)$ and $(qq') = (ud)$ for a $\pi^-$ beam and $(NN') = (np)$ and $(qq') = (du)$ for a $\pi^+$ beam.
These transition GPDs can be related to flavor-diagonal ones by isospin symmetry.


%----------------------------------------------------------------------------------------
% SDHEP frame
%----------------------------------------------------------------------------------------
\begin{figure}[htbp]
	\centering
		\includegraphics[scale=0.5]{diphoton-sdhep-frame.pdf}
	\caption{The frame to analyze the diphoton production process in \eq{eq:diphoton}.
		The $A^*$ represents the collinear quark and antiquark pair attaching the GPD to the hard part.
	}
	\label{fig:frame}
\end{figure}
%----------------------------------------------------------------------------------------

The importance of GPDs lies in the fact that they encode
tomographic parton images in slices of different parton momentum fraction $x$~\citep{Burkardt:2000za, Burkardt:2002hr, Ji:1994av, Ji:1995sv, Lorce:2017xzd, Metz:2020vxd, Ji:1996ek, Polyakov:2002yz, Polyakov:2018zvc, Burkert:2018bqq}. 
For this to be ever possible, we shall be able to precisely extract the $x$ dependence of GPDs.
This turns out to be rather difficult~\cite{Qiu:2022pla, Qiu:2023mrm}, 
because for most of the known processes, when factorizing their amplitudes similarly to \eq{eq:factorize}, 
the GPD convolutions at the leading order (LO) reduce to simple ``scaling'' forms like
\beq[eq:moment]
	F_0(\xi, t) = \int_{-1}^1 dx \frac{F(x, \xi, t) }{x - \xi \pm i \epsilon},
\eeq
which completely integrate over the $x$ dependence.
Inverting the full details of GPDs merely from such moments is an impossible task,
as one can construct an infinite family of analytic solutions $S(x, \xi, t)$ that give zero to \eq{eq:moment}.
These solutions, called shadow GPDs~\cite{Bertone:2021yyz, Moffat:2023svr}, would not be separable from the real GPDs 
if we only had moment-type sensitivity to GPDs like \eq{eq:moment}. 

This scaling property applies to the most well studied processes in the literature, 
including the deeply virtual Compton scattering~\cite{Ji:1996nm, Radyushkin:1997ki, Collins:1998be}, 
deeply virtual meson production~\cite{Brodsky:1994kf, Frankfurt:1995jw, Collins:1996fb}, 
timelike Compton scattering~\cite{Berger:2001xd}, and in particular, 
the exclusive Drell-Yan-type dilepton production~\cite{Berger:2001zn, Goloskokov:2015zsa, Sawada:2016mao},
\beq[eq:dilepton]
	N(p) + \pi(p_2) \to N'(p')+ \gamma^* [\to \ell^-(q_1) + \ell^+(q_2)],
\eeq
which could also be studied at J-PARC to constrain the polarized GPD $\wt{F}$.
In contrast, the diphoton process in \eq{eq:diphoton} overcomes this difficulty and provides enhanced sensitivity to the $x$ dependence of GPDs.
This is because the produced two photons can be radiated from two different parton lines 
that are necessarily linked by a virtual gluon, 
and then this internal gluon propagator carries a large $q_T$ flow to break the LO scaling.
In addition to simple moments like \eq{eq:moment}, the GPD convolutions in \eq{eq:factorize} also involve the special integrals,
\begin{align}
	I[\F^+]
	= \int_{-1}^{1} dx \frac{\F^+(x, \xi, t)}{x - x_p(\theta) + i \epsilon \, \sgn{\cos^2(\theta/2) - z} },
\label{eq:diphoton-special-int}
\end{align}
where $\F^+ = F^+$ or $\wt{F}^+$ is the charge-conjugation-even GPD combination, and the new pole $x_p$ depends on the 
polar angle $\theta$, which is equivalent to $q_T$ for fixed $t$ and $\xi$,
\beq[eq:x-pole]
	x_p(\theta)
		= \xi \bb{ \frac{1 - z + \tan^2(\theta / 2) \, z}{1 - z - \tan^2(\theta / 2) \, z} }.
\eeq
Varying $\theta$ shifts this pole around in the DGLAP region of the GPDs, 
causing an entanglement between the $x$ dependence of GPDs and the observable $\theta$ (or $q_T$) distribution.

%----------------------------------------------------------------------------------------
% SDHEP frame + sensitivity plots
%----------------------------------------------------------------------------------------
\begin{figure}[htbp]
	\centering
		\includegraphics[trim={0 0 -2em 0}, clip, scale=0.5]{diphoton.pdf}
		\includegraphics[trim={-2em -5em 0 0}, clip, scale=0.5]{dilepton.pdf}
	\caption{The $q_T$ distributions for the diphoton [Left; \eq{eq:diphoton}] and dilepton [Right; \eq{eq:dilepton}] production processes, 
		evaluated using different GPD models. For the dilepton process, different GPD models yield the same distribution.
	}
	\label{fig:qt-dist}
\end{figure}
%----------------------------------------------------------------------------------------

Since the $\theta$ dependence cannot be separated from the GPD integrals in \eq{eq:diphoton-special-int},
it does not seem possible to construct a shadow GPD that gives zero to \eq{eq:diphoton-special-int} for all $\theta$ values.
The diphoton process can therefore distinguish the real and shadow GPDs (for the specific flavor transition), at least in principle.
To demonstrate the numerical effects, we take the Goloskokov-Kroll model~\cite{Goloskokov:2005sd, Goloskokov:2007nt, Goloskokov:2009ia, Kroll:2012sm} 
as the base GPDs $(H_0, \wt{H}_0)$,
and vary either $H_0$ or $\wt{H}_0$ by adding analytically constructed shadow GPDs to construct $(H_1, H_2, H_3)$ and $(\wt{H}_1, \wt{H}_2)$.
Taking these models, we calculate the differential cross sections for both processes in Eqs.~\eqref{eq:diphoton} and \eqref{eq:dilepton},
which are illustrated in \fig{fig:qt-dist} as distributions of $q_T$. 
Clearly, these different models yield different distributions for the diphoton process, in terms of both shape and magnitude.
The sensitivity to the polarized GPD $\wt{H}$ is higher than the unpolarized one $H$.
In contrast, since the shadow GPDs give zero contribution to \eq{eq:moment} by definition, these models are not separable by the dilepton process.
Furthermore, it is evident that the diphoton process also yields a higher rate than the dilepton one.

In conclusion, the exclusive diphoton production process offers J-PARC a novel and exceptional opportunity to explore the GPDs, especially their $x$ dependence. 
Realizing this potential could bring us significantly closer to obtaining the tomographic image of the proton.

